Spatial profiles of a reaction-diffusion epidemic model with nonlinear incidence mechanism and constant total population

This paper examines a susceptible-infected-susceptible (SIS) epidemic reaction-diffusion model with no-flux boundary conditions and constant total population. The infection mechanism in the model is described by a nonlinear term of the form $S^qI^p$ with $0<p\leq1$ and $q>0$. We explore the spatial profiles of the endemic equilibrium with respect to small movement rates of susceptible and/or infected populations. Our results extend and improve existing results in the literature, providing further insights into how transmission mechanisms and population mobility limitations impact the spread of infectious diseases. We reinforce and complement the theoretical results with numerical simulations.

==> ex_shared1.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Spatial profiles of a diffusive epidemic model}{P. Rui, R. Salako, and Y. Wu}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Spatial profiles of  a reaction-diffusion epidemic model with nonlinear incidence mechanism and constant total population \thanks{Submitted to the editors DATE.
\funding{R. Peng was partially supported by NSF of China (No. 12271486, 12171176).}}}

% Authors: full names plus addresses.
\author{Rui Peng\thanks{School of Mathematical Sciences, Zhejiang Normal
University, Jinhua, 321004, Zhejiang, China 
  (\email{pengrui\_seu@163.com}).}
\and Rachidi Salako\thanks{Department of Mathematical Sciences, University of Nevada Las Vegas, Las Vegas, NV 89154, USA 
  (\email{rachidi.salako@unlv.edu}).}
\and Yixiang Wu\thanks{ Department of Mathematical Sciences, Middle Tennessee State University, Murfreesboro, TN 37132, USA 
  (\email{yixiang.wu@mtsu.edu}).}}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> ex_shared2.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Spatial profiles of solutions to a diffusive epidemic model}{P. Rui, R. Salako, and Y. Wu}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Spatial profiles of solutions to a reaction-diffusion epidemic model with nonlinear incidence mechanism and varying total population\thanks{Submitted to the editors DATE.
\funding{R. Peng was partially supported by NSF of China (No. 12271486, 12171176).}}}

% Authors: full names plus addresses.
\author{Rui Peng\thanks{School of Mathematical Sciences, Zhejiang Normal
University, Jinhua, 321004, Zhejiang, China 
  (\email{pengrui\_seu@163.com}).}
\and Rachidi Salako\thanks{Department of Mathematical Sciences, University of Nevada Las Vegas, Las Vegas, NV 89154, USA 
  (\email{rachidi.salako@unlv.edu}).}
\and Yixiang Wu\thanks{ Department of Mathematical Sciences, Middle Tennessee State University, Murfreesboro, TN 37132, USA 
  (\email{yixiang.wu@mtsu.edu}).}}
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

